Aperture-corrected spectroscopic type Ia supernova host galaxy properties

We use type Ia supernovae (SNe Ia) data obtained by the Sloan Digital Sky Survey-II Supernova Survey (SDSS-II/SNe) in combination with the publicly available SDSS DR16 fiber spectroscopy of their host galaxies to correlate SNe Ia light-curve parameters and Hubble residuals to several host galaxy properties. Fixed-aperture fiber spectroscopy suffers from aperture effects: the fraction of the galaxy covered by the fiber varies depending on its projected size on the sky, thus measured properties are not representative of the whole galaxy. The advent of Integral Field Spectroscopy has provided a way for correcting the missing light, by studying how these galaxy parameters change with the aperture size. Here we study how the standard SN host galaxy relations change once global host galaxy parameters are corrected for aperture effects. We recover previous trends on SN Hubble residuals with host galaxy properties, but we find that discarding objects with poor fiber coverage instead of correcting for aperture loss introduces biases in the sample that affect SN host galaxy relations. The net effect of applying the commonly used $g$-band fraction criterion is discarding intrinsically faint \mbox{SNe~Ia} in high-mass galaxies, thus artificially increasing the height of the mass step by 0.02 mag and its significance. Current and next generation of fixed-aperture fiber spectroscopy surveys, such as DES, DESI or TiDES in 4MOST, that aim at study SN and galaxy correlations must consider, and correct for, these effects.

==> hostdiff.tex <==
\begin{table}[h!] \small
\caption{Host galaxies changed from the SDSS-II/SNe Survey Data Release.}
\begin{center}
\begin{tabular}{lccl}
SN ID & Galaxy in DR & Galaxy this work & Reason\\
\hline \hline
904 & 1237657190914457965 & 1237657190914457964 & FAINT \\
1580 & 1237663783143473374 & 1237663783143473373 & OTHER \\
2064 & 1237663457242186614 & 1237663457242186612 & FAINT \\
%2308 & --- & 1237666408457437617 & FAIL (?)\\ %redshift 0.148 to 0.272  MANU NOOO    45% 
4046 & 1237657191976534239 & 1237657191976534238 & FAINT \\ % redshift 0.277 to 0.286     3%
%4241 & 1237657189836849751 & 1237657189836849748 & FAINT(?) \\ %redshift 0.332 to 0.366 MANU NOOO   9%
4612 & 1237663783129580009 & 1237663783129580008 & FAINT \\
%6924 & --- & 1237663278464172544 & FAIL (? - ?) \\ % redshift 0.328 to 0.273   20%
7051 & 1237663784196767937 & 1237663784196767936 & OTHER \\
8888 & 1237657191444316872 & 1237657191444316871 & FAINT \\
12136 &1237663783656161962 & 1237663783656161959 & FAINT \\
13344 & 1237663543685546296 & 1237663543685546294 & BETTER \\
13903 & 1237666408442298652 & 1237666408442298654 & OTHER \\ %redsghift 0.263 to 0.253 MANU NOO  4%
15103 & 1237663542612656918 & 1237663542612656919 & OTHER \\
%15674 & --- & 1237663543687578404 & FAIL (? - ?) \\  %redshift 0.198 to 0.235  15%
16626 & 1237663783127613910 & 1237663783127613911 & OTHER \\
%16793 & --- & 1237663479793582771 &FAIL (? - ?) \\  %redshift 0.222 to 0.263  15%
18945 & --- & 1237657189835866770 &FAIL \\
20345 & --- & 1237657191446741848 &FAIL \\
20578 & 1237663479257170514 & 1237663479257170513 & BETTER \\ 
\end{tabular}
\end{center}
\label{tab:coord}
\end{table}

==> qso.tex <==
\begin{table}[h!]
\caption{Host galaxies containing QSOs.}
\begin{center}
\begin{tabular}{lc}
SN ID & Galaxy ID in DR \\
\hline
   5966  & 1237663784741372369 \\
   15041 & 1237666407918338758 \\
   15272 & 1237663784193360056 \\
   15988 & 1237663784206533181 \\
   18283 & 1237657070090781290 \\
   18782 & 1237657584949789257 \\
   18827 & 1237678437015552153 \\
   19778 & 1237666407364165976 \\
   20245 & 1237663544224842023 \\
   20745 & 1237666408441840260 \\
   21150 & 1237657192515502214 \\
   21502 & 1237656906352296084 \\
   21878 & 1237678437017583918 \\
\end{tabular}
\end{center}
\label{tab:qso}
\end{table}

==> tab1.tex <==
\begin{table*}[!t]
\caption{Results of the {\sc LINMIX} MCMC slopes, and difference (steps) between the high and low bin.}
\begin{center}
\begin{tabular}{llcccccc}
\hline
         &            &            c     & $\sigma$ &          x1      & $\sigma$ &          HR      & $\sigma$ \\ 
\hline
\multicolumn{8}{c}{log (Mass [M$_\odot$])}\\
\hline
%Ap. cor. & slope   &  0.003$\pm$0.007 & 0.50 & -0.255$\pm$0.073 & 3.48 & -0.062$\pm$0.017 & 3.59 \\
%         & step    &  0.016$\pm$0.010 & 1.63 & -0.263$\pm$0.096 & 2.74 & -0.096$\pm$0.025 & 3.91 \\
%g-frac   & slope   &  0.002$\pm$0.008 & 0.29 & -0.304$\pm$0.090 & 3.38 & -0.101$\pm$0.022 & 4.68 \\
%         & step    &  0.013$\pm$0.010 & 1.30 & -0.265$\pm$0.107 & 2.48 & -0.118$\pm$0.028 & 4.23 \\
Ap. cor. & slope   &  0.004$\pm$0.007 & 0.50 & -0.249$\pm$0.071 & 3.49 & -0.064$\pm$0.017 & 3.75 \\
         & step    & -0.012$\pm$0.009 & 1.34 &  0.223$\pm$0.092 & 2.43 &  0.078$\pm$0.022 & 3.60 \\
g-frac   & slope   &  0.003$\pm$0.009 & 0.34 & -0.299$\pm$0.085 & 3.53 & -0.104$\pm$0.022 & 4.73 \\
         & step    & -0.011$\pm$0.010 & 1.11 &  0.239$\pm$0.107 & 2.24 &  0.097$\pm$0.026 & 3.78 \\

\hline
\multicolumn{8}{c}{12 + log (O/H)$_{03N2}$}\\
\hline
%Ap. cor. & slope   &  0.029$\pm$0.033 & 0.88 & -0.569$\pm$0.347 & 1.64 & -0.188$\pm$0.071 & 2.60 \\
%         & step    &  0.007$\pm$0.009 & 0.72 & -0.203$\pm$0.093 & 2.19 & -0.054$\pm$0.023 & 2.37 \\
%g-frac   & slope   &  0.050$\pm$0.037 & 1.37 & -0.612$\pm$0.379 & 1.62 & -0.263$\pm$0.081 & 3.26 \\
%         & step    &  0.018$\pm$0.010 & 1.84 & -0.197$\pm$0.106 & 1.86 & -0.068$\pm$0.027 & 2.52 \\
Ap. cor. & slope   &  0.031$\pm$0.033 & 0.93 & -0.558$\pm$0.328 & 1.70 & -0.182$\pm$0.076 & 2.39 \\
         & step    & -0.004$\pm$0.009 & 0.48 &  0.177$\pm$0.092 & 1.92 &  0.033$\pm$0.022 & 1.49 \\
g-frac   & slope   &  0.053$\pm$0.036 & 1.46 & -0.597$\pm$0.375 & 1.59 & -0.243$\pm$0.082 & 2.96 \\
         & step    & -0.019$\pm$0.010 & 1.86 &  0.153$\pm$0.105 & 1.46 &  0.051$\pm$0.026 & 1.96 \\

\hline
\multicolumn{8}{c}{log (sSFR [yr$^{-1}$])}\\
\hline
%Ap. cor. & slope   & -0.004$\pm$0.007 & 0.62 &  0.391$\pm$0.065 & 6.02 &  0.056$\pm$0.015 & 3.71 \\
%         & step    & -0.003$\pm$0.009 & 0.34 &  0.294$\pm$0.092 & 3.20 &  0.094$\pm$0.022 & 4.32 \\
%g-frac   & slope   & -0.006$\pm$0.008 & 0.76 &  0.532$\pm$0.078 & 6.80 &  0.079$\pm$0.019 & 4.28 \\
%         & step    & -0.010$\pm$0.010 & 0.99 &  0.388$\pm$0.104 & 3.73 &  0.094$\pm$0.026 & 3.64 \\
Ap. cor. & slope   & -0.004$\pm$0.007 & 0.60 &  0.383$\pm$0.069 & 5.55 &  0.056$\pm$0.015 & 3.76 \\
         & step    &  0.002$\pm$0.009 & 0.25 & -0.284$\pm$0.092 & 3.09 & -0.092$\pm$0.022 & 4.24 \\
g-frac   & slope   & -0.007$\pm$0.008 & 0.81 &  0.520$\pm$0.082 & 6.30 &  0.077$\pm$0.019 & 4.04 \\
         & step    &  0.014$\pm$0.010 & 1.42 & -0.328$\pm$0.104 & 3.14 & -0.093$\pm$0.026 & 3.59 \\
\hline
\multicolumn{8}{c}{log (H$\alpha$ EW [$\AA$])}\\
\hline
%Ap. cor. & slope   & -0.002$\pm$0.009 & 0.18 &  0.586$\pm$0.092 & 6.40 &  0.061$\pm$0.026 & 2.37 \\
%         & step    & -0.008$\pm$0.009 & 0.88 &  0.355$\pm$0.092 & 3.86 &  0.086$\pm$0.022 & 3.99 \\
%g-frac   & slope   & -0.004$\pm$0.009 & 0.46 &  0.619$\pm$0.094 & 6.59 &  0.086$\pm$0.024 & 3.55 \\
%         & step    & -0.008$\pm$0.010 & 0.81 &  0.458$\pm$0.105 & 4.35 &  0.100$\pm$0.026 & 3.93 \\
Ap. cor. & slope   & -0.002$\pm$0.009 & 0.26 &  0.582$\pm$0.089 & 6.56 &  0.073$\pm$0.020 & 3.64 \\
         & step    &  0.011$\pm$0.009 & 1.15 & -0.385$\pm$0.091 & 4.21 & -0.086$\pm$0.022 & 3.92 \\
g-frac   & slope   & -0.003$\pm$0.009 & 0.36 &  0.625$\pm$0.088 & 7.14 &  0.093$\pm$0.023 & 4.10 \\
         & step    &  0.003$\pm$0.010 & 0.34 & -0.522$\pm$0.104 & 5.03 & -0.107$\pm$0.026 & 4.19 \\
\hline
\end{tabular}
\end{center}
\label{tab:res}
\end{table*}

